The Fragility of Sparsity

We show, using three empirical applications, that linear regression estimates predicated on the assumption of sparsity are fragile in two ways. First, we document that different choices of the regressor matrix which do not impact ordinary least squares (OLS) estimates, such as the choice of baseline category with categorical controls, can move sparsity-based estimates by two standard errors or more. Second, we develop two tests of the sparsity assumption by comparing sparsity-based estimators with OLS. The tests tend to reject the sparsity assumption in all three applications. Unless the number of regressors is comparable to or exceeds the sample size, OLS yields more robust inference at little efficiency cost.

==> replication_t1.tex <==
Percentage & 52.7 & 62.2 & 97.1 & 23.7\\
Number of papers & 35 & 35 & 35 & 47\\


==> replication_t2.tex <==
Percentage & 54.4 & 63.6 & 95.8 & 21.4\\
Number of papers & 24 & 24 & 24 & 24\\


==> table1.tex <==
\multicolumn{7}{@{}c}{{A\@: BCH}}\\
$\Delta\ln(\text{violent crime/capita})$ & 0.006 & -0.160 & -0.216 & -0.109 & -0.160 & -0.122\\
($n=576$, $p=294$) & (0.755) & (0.112) & (0.118) & (0.093) & (0.112) & (0.097)\\
$\Delta\ln(\text{property crime/capita})$ & -0.154 & -0.110 & -0.137 & -0.054 & -0.127 & -0.078\\
($n=576$, $p=294$) & (0.223) & (0.045) & (0.045) & (0.047) & (0.038) & (0.041)\\
$\Delta\ln(\text{murder/capita})$ & 2.240 & -0.131 & -0.225 & -0.061 & -0.149 & -0.066\\
($n=576$, $p=294$) & (2.819) & (0.146) & (0.140) & (0.149) & (0.151) & (0.161)\\[1ex]
\multicolumn{7}{@{}c}{{B\@: \textcite{ferrara22}}}\\
\% Semiskilled Black workers & 0.118 & 0.548 & 0.242 & 0.657 & 0.482 & 0.548\\
($n=4,903$, $p=2,252$) & (0.126) & (0.167) & (0.126) & (0.153) & (0.137) & (0.167)\\[1ex]
\multicolumn{7}{@{}c}{{C\@: \textcite{enke20}}}\\
Trump $-$ avg.~GOP & -3.676 & -1.921 & -2.120 & -1.840 &  & \\
($n=2,452$, $p=978$) & (1.416) & (0.941) & (0.950) & (0.934) &  & \\
Voted for Trump in 2016 & -12.399 & -12.335 & -12.357 & -11.955 &  & \\
($n=2,852$, $p=1,068$) & (1.357) & (1.050) & (1.049) & (1.028) &  & \\
Voted for Trump in primaries & -5.318 & -7.778 & -8.618 & -7.716 &  & \\
($n=1,544$, $p=824$) & (2.660) & (1.544) & (1.534) & (1.541) &  & \\


==> table2.tex <==
\multicolumn{5}{@{}c}{{A\@: BCH}}\\
$\Delta\ln(\text{violent crime/capita})$ &  &  & -0.239 & 0.107\\
($n=576$, $p=294$) &  &  & (0.105) & (0.093)\\
$\Delta\ln(\text{property crime/capita})$ &  &  & -0.193 & -0.011\\
($n=576$, $p=294$) &  &  & (0.047) & (0.053)\\
$\Delta\ln(\text{murder/capita})$ &  &  & -0.338 & 0.128\\
($n=576$, $p=294$) &  &  & (0.160) & (0.195)\\[1ex]
\multicolumn{5}{@{}c}{{B\@: \textcite{ferrara22}}}\\
\% Semiskilled Black workers & 0.401 & 0.685 & 0.397 & 0.646\\
($n=4,903$, $p=2,252$) & (0.134) & (0.162) & (0.148) & (0.164)\\[1ex]
\multicolumn{5}{@{}c}{{C\@: \textcite{enke20}}}\\
Trump $-$ avg.~GOP & -2.333 & -1.476 &  & \\
($n=2,452$, $p=978$) & (0.918) & (0.906) &  & \\
Voted for Trump in 2016 & -12.946 & -11.202 &  & \\
($n=2,852$, $p=1,068$) & (1.029) & (1.008) &  & \\
Voted for Trump in primaries & -9.269 & -7.083 &  & \\
($n=1,544$, $p=824$) & (1.526) & (1.525) &  & \\


==> table3.tex <==
\multicolumn{11}{@{}c}{{A\@: BCH}}\\
$\Delta\ln(\text{violent}$ & H & 81.7 & 76.0 & 87.4 & 81.7 & 85.8 &  &  & 73.1 & 100.0\\
$\text{crime/capita})$ & OR & 9.5 & 9.5 & 9.5 & 9.5 & 9.5 &  &  & 8.2 & 20.2\\
 & PR & 0.3 & 0.0 & 0.9 & 0.0 & 0.6 &  &  & 0.0 & 2.2\\
$\Delta\ln(\text{property}$ & H & 82.6 & 61.8 & 93.4 & 70.9 & 89.7 &  &  & 47.5 & 100.0\\
$\text{crime/capita})$ & OR & 12.0 & 12.0 & 12.0 & 12.0 & 12.0 &  &  & 10.4 & 45.4\\
 & PR & 28.8 & 12.6 & 35.0 & 0.0 & 29.9 &  &  & 0.0 & 39.9\\
$\Delta\ln(\text{murder/}$ & H & 21.0 & 19.7 & 22.5 & 20.4 & 22.6 &  &  & 17.3 & 26.8\\
$\text{capita})$ & OR & 43.3 & 43.3 & 43.3 & 43.3 & 43.3 &  &  & 43.3 & 45.4\\
 & PR & 0.4 & 0.2 & 1.1 & 0.4 & 1.2 &  &  & 0.0 & 26.0\\[1ex]
\multicolumn{11}{@{}c}{{B\@: \textcite{ferrara22}}}\\
\% Semiskilled & H & 0.0 & 0.0 & 5.5 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
Black workers & OR & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
 & PR & 34.5 & 19.6 & 49.7 & 34.5 & 53.3 & 11.0 & 96.6 & 34.7 & 73.3\\[1ex]
\multicolumn{11}{@{}c}{{C\@: \textcite{enke20}}}\\
Trump $-$ & H & 6.1 & 4.9 & 9.5 &  &  & 1.8 & 15.2 &  & \\
avg.~GOP & OR & 13.0 & 5.1 & 13.0 &  &  & 5.0 & 30.3 &  & \\
 & PR & 0.2 & 0.1 & 0.2 &  &  & 0.0 & 4.0 &  & \\
Voted for Trump & H & 94.6 & 63.1 & 96.4 &  &  & 19.0 & 100.0 &  & \\
in 2016 & OR & 0.0 & 0.0 & 0.5 &  &  & 0.0 & 14.1 &  & \\
 & PR & 0.1 & 0.0 & 0.1 &  &  & 0.0 & 1.4 &  & \\
Voted for Trump & H & 15.5 & 5.9 & 16.6 &  &  & 2.6 & 30.5 &  & \\
in primaries & OR & 9.6 & 2.8 & 9.6 &  &  & 0.7 & 40.6 &  & \\
 & PR & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0.6 &  & \\


==> table4.tex <==
\multicolumn{6}{@{}c}{{A\@: BCH}}\\
$\Delta\ln(\text{violent}$ & H & 5.5 & 5.6 & 5.1 & 5.1\\
$\text{crime/capita})$ & PR & 1.8 & 1.8 & 1.5 & 1.5\\
 & OR & 1.7 & 1.7 & 1.6 & 1.6\\
$\Delta\ln(\text{property}$ & H & 4.9 & 4.9 & 5.6 & 5.5\\
$\text{crime/capita})$ & PR & 1.7 & 1.7 & 1.6 & 1.6\\
 & OR & 1.7 & 1.7 & 1.5 & 1.5\\
$\Delta\ln(\text{murder/}$ & H & 5.4 & 5.4 & 4.9 & 5.0\\
$\text{capita})$ & PR & 1.6 & 1.6 & 1.6 & 1.6\\
 & OR & 1.8 & 1.8 & 1.7 & 1.7\\[1ex]
\multicolumn{6}{@{}c}{{B\@: \textcite{ferrara22}}}\\
\% Semiskilled & H & 4.9 & 4.8 & 5.1 & 5.1\\
Black workers & PR & 3.9 & 4.2 & 3.9 & 4.2\\
 & OR & 4.1 & 4.4 & 4.1 & 4.4\\[1ex]
\multicolumn{6}{@{}c}{{C\@: \textcite{enke20}}}\\
Trump $-$ & H & 5.1 & 5.0 & 5.2 & 5.2\\
avg.~GOP & PR & 3.0 & 4.6 & 3.3 & 5.0\\
 & OR & 3.2 & 4.8 & 3.3 & 4.9\\
Voted for Trump & H & 5.1 & 5.1 & 4.9 & 4.8\\
in 2016 & PR & 3.1 & 4.8 & 3.2 & 4.9\\
 & OR & 3.3 & 4.8 & 3.3 & 4.8\\
Voted for Trump & H & 5.1 & 5.0 & 5.0 & 5.1\\
in primaries & PR & 3.1 & 4.5 & 3.3 & 5.0\\
 & OR & 3.2 & 4.7 & 3.2 & 4.8\\

